Some Essential Constructive Foundations for Systems and Control

This work develops several constructive foundations for systems and control within Bishop-style constructive mathematics. For an engineer, the guiding principle is that an object claimed to exist, such as a trajectory, an optimal control law, a selector, or a viable solution, should come with finite data and an operation computing approximations to any prescribed precision. The style remains close to classical analysis, but existential statements are organized so that their computational content is visible. The paper begins with elementary geometric data in finite-dimensional Euclidean spaces: blocks, multiblocks, representable sets, regular functions, and certified integrals. This set-first integration route is meant to complement, rather than replace, abstract constructive integration theories such as Daniell-type or integration-space approaches. The developed apparatus is then applied to a constructive functional extremum-value theorem, selector extraction for multifunctions, Filippov-type and viable solutions of differential inclusions, regular probability densities, controlled Markov chains, and empirical density certificates. A short account of resolvent projectors and linear stability is included for completeness.

==> input/intro.tex <==
\section{Chan Integration-Space Comparison}
\label{app_chan_integration_space}

\begin{definition}[Integration space]
	\label{dfn_integrable_space}
	An \emph{integration space} is a triple
	\[
		\left(\Omega,\mathcal L,\int_\Omega\right)
	\]
	where $\Omega$ is a nonempty set, $\mathcal L$ is a set of real-valued functions whose domains are subsets of $\Omega$, and $\int_\Omega:\mathcal L\to\R$ is a nonzero functional with domain $\mathcal L$, satisfying the following conditions.
	Pointwise operations are understood on their natural domains; for example, $af+bg$ is defined on $\dom{f}\cap\dom{g}$.
	\begin{enumerate}
		\item If $f,g\in\mathcal L$ and $a,b\in\R$, then
		\[
			af+bg,\qquad |f|,\qquad f\land1
		\]
		belong to $\mathcal L$, and
		\[
			\int_\Omega(af+bg)
			=
			a\int_\Omega f+b\int_\Omega g.
		\]
		\item If $f_0,f_1,f_2,\ldots\in\mathcal L$, if $f_i\ge0$ for each $i\ge1$, and if
		\[
			\sum_{i=1}^\infty \int_\Omega f_i
			<
			\int_\Omega f_0,
		\]
		then there exists
		\[
			\omega\in\bigcap_{i=0}^{\infty}\dom{f_i}
		\]
		such that
		\[
			\sum_{i=1}^\infty f_i(\omega)<f_0(\omega).
		\]
		\item For each $f\in\mathcal L$,
		\[
			\int_\Omega (f\land n)\to\int_\Omega f,
			\qquad
			\int_\Omega (|f|\land n^{-1})\to0
		\]
		as $n\to\infty$ through positive integers.
	\end{enumerate}
	A function in $\mathcal L$ is called \emph{integrable} relative to $\int_\Omega$.
\end{definition}

\begin{remark}
	\label{rem_integrable_space_chan}
	This is Chan's scalar integration-space definition, written with the symbol $\int$ instead of a separate letter for the functional \cite{Chan2019FoundationsCon}.
	The definition is scalar: the order, absolute value, truncation, and positivity condition are all statements about real-valued functions.
\end{remark}

\begin{definition}[Vector-valued integration module]
	\label{dfn_vector_valued_integration_module}
	Let $\left(\Omega,\mathcal L,\int_\Omega\right)$ be an integration space and let $m\in\N$ be positive.
	Set
	\[
		\mathcal L^m:=
		\left\{
			F=(F_1,\ldots,F_m):F_j\in\mathcal L,\ j=1,\ldots,m
		\right\}.
	\]
	An element $F=(F_1,\ldots,F_m)$ is regarded as an $\R^m$-valued function on the common domain $\bigcap_{j=1}^m\dom{F_j}$.
	For $F\in\mathcal L^m$, define
	\[
		\int_\Omega F
		:=
		\left(
			\int_\Omega F_1,\ldots,\int_\Omega F_m
		\right)
		\in\R^m.
	\]
	The pair $\left(\mathcal L^m,\int_\Omega\right)$, with the integral symbol understood componentwise, is called the $m$-dimensional integration module over $\left(\Omega,\mathcal L,\int_\Omega\right)$.
\end{definition}

\begin{remark}
	\label{rem_vector_integration_componentwise}
	For $m>1$ we do not modify \Cref{dfn_integrable_space}.
	There is no canonical lattice order on $\R^m$, so Chan's positivity axiom remains scalar.
	Vector-valued regular functions are integrated componentwise; equivalently, every scalar linear observable of a vector-valued integrable function is integrable.
\end{remark}

\begin{lemma}[Finite positivity]
	\label{lem_regular_finite_sum_positivity}
	Let $B$ be a full block.
	Let $f_0,f_1,\ldots,f_N\in\BReg{B}$, and let $f_i\ge0$ for $i=1,\ldots,N$.
	If
	\[
		\sum_{i=1}^N\int_B f_i
		<
		\int_B f_0,
	\]
	then there exists $x\in B$ such that
	\[
		\sum_{i=1}^N f_i(x)<f_0(x).
	\]
\end{lemma}

\begin{proof}
	Set
	\[
		h:=f_0-\sum_{i=1}^N f_i.
	\]
	By \Cref{lem_regular_functions_finite_algebra}, $h$ is regular and
	\[
		\int_Bh>0.
	\]
	Choose a rational $\alpha>0$ with $\alpha<\int_Bh$.
	Since $h$ is Riemann integrable, choose a tagged multiblock $\mathcal P$ with
	\[
		\abs{\Sigma(h,\mathcal P)-\int_Bh}<\alpha/2.
	\]
	Then $\Sigma(h,\mathcal P)>\alpha/2$.
	The sum defining $\Sigma(h,\mathcal P)$ is finite.
	If every tag $\xi$ of $\mathcal P$ satisfied $h(\xi)\le0$, then $\Sigma(h,\mathcal P)\le0$, a contradiction.
	Therefore one tag satisfies $h(\xi)>0$, which is the required point.
\end{proof}

\begin{lemma}[Ye bisection positivity for regular functions]
	\label{lem_ye_bisection_regular_positivity}
	Let $B$ be a full block.
	Let $f_0,f_1,f_2,\ldots\in\BReg{B}$, and let $f_i\ge0$ for $i\ge1$.
	If
	\[
		\sum_{i=1}^\infty\int_B f_i
		<
		\int_B f_0,
	\]
	then there exists $\omega\in B$ such that
	\[
		\sum_{i=1}^\infty f_i(\omega)<f_0(\omega).
	\]
\end{lemma}

\begin{proof}
	The proof is the dyadic bisection and doubling construction of Ye's \cite[Lemma~6.1]{Ye2011StrictFinitism}, with trimmed coordinate refinements inserted to handle the finite support boundaries of regular functions.
	Set
	\[
		F:=f_0\lor0.
	\]
	The function $F$ is regular by \Cref{cor_regular_functions_lattice_closure}.
	Since $F\ge f_0$ and $f_i\ge0$, the number
	\[
		\eta
		:=
		\int_B F
		-
		\sum_{i=1}^\infty\int_B f_i
	\]
	is positive.
	Choose $\eps>0$ so small that
	\[
		\eps\mu(B)<\eta/2,
	\]
	and let $h_\eps$ be the constant function $\eps$ on $B$.
	It is enough to construct $\omega\in B$ with
	\[
		h_\eps(\omega)
		+
		\sum_{i=1}^\infty f_i(\omega)
		\le
		F(\omega).
	\]
	Indeed, then $F(\omega)>0$, hence $F(\omega)=f_0(\omega)$, and the desired strict inequality follows.
	For a full subblock $Q\subseteq B$ write
	\[
		\Delta_Q(g;(g_i)_{i\ge1})
		:=
		\int_Q g
		-
		\sum_{i=1}^\infty\int_Q g_i.
	\]
	The restrictions to such $Q$ are integrated by the same tagged-multiblock Riemann construction as on $B$.
	Starting from the positive gap
	\[
		\Delta_B(F;(h_\eps,f_1,f_2,\ldots))>0,
	\]
	construct nested full blocks
	\[
		B\supset Q_1\supset Q_2\supset\cdots
	\]
	with $\diam(Q_k)\to0$ and
	\[
		\Delta_{Q_k}(F;(h_\eps,f_1,f_2,\ldots))>0.
	\]
	At the $k$th step, take representability witnesses for the finitely many supports occurring in
	\[
		F,\quad h_\eps,\quad f_1,\ldots,f_{k+1}
	\]
	with total exception cost small compared with the current positive gap.
	Apply the trimmed coordinate refinement inside $Q_k$.
	The exception and coordinate-boundary cells remove less than half of the gap, so the finite sum of the gaps over the remaining trimmed cells is still positive.
	A finite search through those cells gives $Q_{k+1}$ with positive gap.
	The refinement is chosen thin enough that $Q_{k+1}$ also fixes the branch data of $F,h_\eps,f_1,\ldots,f_{k+1}$.
	The nested blocks determine a point $\omega\in B$.
	For every fixed $N$, the functions $F,h_\eps,f_1,\ldots,f_N$ are continuous on all sufficiently late $Q_k$ with fixed branches.
	The positive gap on such a $Q_k$ gives a tag $\xi_k\in Q_k$ with
	\[
		h_\eps(\xi_k)
		+
		\sum_{i=1}^N f_i(\xi_k)
		<
		F(\xi_k).
	\]
	Letting $k\to\infty$ gives
	\[
		h_\eps(\omega)
		+
		\sum_{i=1}^N f_i(\omega)
		\le
		F(\omega)
	\]
	for every $N$.
	Choose indices $N_j$ such that
	\[
		\sum_{i=N_j}^\infty\int_B f_i<2^{-j}\eta/4.
	\]
	Apply the same construction to Ye's rearranged sequence
	\[
		h_\eps,\quad
		f_1,\quad
		2\sum_{i=N_1}^{N_2-1}f_i,\quad
		f_2,\quad
		2^2\sum_{i=N_2}^{N_3-1}f_i,\quad
		f_3,\ldots .
	\]
	Its integral sum is still strictly below $\int_BF$.
	The finite-partial-sum conclusion for this rearranged sequence gives
	\[
		\sum_{i=N_j}^{N_{j+1}-1}f_i(\omega)
		\le
		2^{-j}F(\omega).
	\]
	Thus the value series $\sum_i f_i(\omega)$ converges, and the finite-partial-sum inequalities pass to
	\[
		h_\eps(\omega)
		+
		\sum_{i=1}^\infty f_i(\omega)
		\le
		F(\omega).
	\]
\end{proof}

\begin{remark}[Tails in the Ye construction]
	\label{rem_ye_tail_control_limit_point}
	The amplified-tail step in \Cref{lem_ye_bisection_regular_positivity} controls the tail only at the final limit point $\omega$.
	It does not provide a finite stage $x_k$ at which the full infinite tail is already certified.
	Such a finite stopping statement requires extra pointwise tail data, for instance a summable uniform bound $0\le f_i(x)\le M_i$ with a known convergence modulus for $\sum_iM_i$.
\end{remark}

\begin{theorem}[Regular functions as an integration space]
	\label{thm_regular_functions_integration_space}
	Let $B$ be a full block.
	The triple
	\[
		\left(B,\BReg{B},\int_B\right)
	\]
	is an integration space in the sense of \Cref{dfn_integrable_space}.
\end{theorem}

\begin{proof}
	The functional is nonzero because every full block contains a smaller full block $A\Subset B$, and the representable indicator $\indic{A}$ satisfies $\int_B\indic{A}=\mu(A)>0$.
	Linearity and finite order are \Cref{lem_regular_functions_finite_algebra,lem_regular_integral_finite_order}.
	The lattice operations $|f|$ and $f\land1$ are obtained from \Cref{cor_regular_functions_lattice_closure}.
	Chan's countable positivity axiom is \Cref{lem_ye_bisection_regular_positivity}.
	The truncation axiom follows from boundedness.
	Indeed, for each $f\in\BReg{B}$ and for $n$ larger than a bound witness for $f$ one has $f\land n=f$, while
	\[
		0
		\le
		\int_B(|f|\land n^{-1})
		\le
		n^{-1}\mu(B)
		\to0.
	\]
	Since every member of $\BReg{B}$ is Riemann integrable by \Cref{lem_regular_functions_riemann_integrable}, these axioms restrict to $\BReg{B}$.
\end{proof}

\begin{corollary}[Vector-valued regular integration module]
	\label{crl_vector_regular_integration_module}
	Let $B$ be a full block.
	For every positive $m\in\N$, the $\R^m$-valued effectively bounded regular functions on $B$ whose supports are well contained in $B$ form the componentwise integration module over the scalar integration space in \Cref{thm_regular_functions_integration_space}.
\end{corollary}

\begin{proof}
	This is \Cref{dfn_vector_valued_integration_module} applied to \Cref{thm_regular_functions_integration_space}.
\end{proof}

